A Simulation Framework for Ride-Hailing with Electric Vehicles

This research presents a Python-based simulation framework designed to model electric vehicle (EV) on-demand transportation systems, with a focus on optimizing urban fleet operations. Built on a process-driven architecture, the system efficiently simulates EV fleet dynamics, including passenger matching, vehicle dispatching, and charging strategies, while enabling customization to address critical challenges such as charger placement, fleet management, and algorithm performance. We overcome the challenge of high dimensional state-space and non-Markovian system dynamics by executing processes asynchronously using SimPy and updating only the states that are affected by employing object-oriented programming. As a result, our simulation framework is capable of handling peak demand scenarios involving thousands of trips and completing multi-day scenarios in minutes. The modular design enables users to experiment with parameters, test algorithms, and integrate custom datasets, making the tool highly adaptable for diverse urban contexts. By providing a realistic and extensible platform, this adaptable, scalable, and open-source framework advances the optimization of EV fleet operations and offers a valuable resource for decision-makers and city planners navigating the transition to sustainable urban mobility solutions. We also present a case study using the NYC taxi dataset evaluating various dispatching algorithms, including closest vehicle dispatch, closest available vehicle dispatch, and power-of-d vehicle dispatch, and exploring charging approaches like continuous and nighttime charging. We propose a novel adaptive power-of-d dispatch policy, which dynamically adjusts to real-time conditions and demonstrates high throughputs when combined with adaptive charging policies that interrupt charging to meet demand during the peak and delay some of the charging to the nighttime.

==> howto.tex <==
\subsection{How to include Figures}

First you have to upload the image file from your computer using the upload link the project menu. Then use the includegraphics command to include it in your document. Use the figure environment and the caption command to add a number and a caption to your figure. See the code for Figure \ref{fig:frog} in this section for an example.

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{frog.jpg}
\caption{\label{fig:frog}This frog was uploaded via the project menu.}
\end{figure}

\subsection{How to add Comments}

Comments can be added to your project by clicking on the comment icon in the toolbar above. % * <john.hammersley@gmail.com> 2016-07-03T09:54:16.211Z:
%
% Here's an example comment!
%
To reply to a comment, simply click the reply button in the lower right corner of the comment, and you can close them when you're done.

Comments can also be added to the margins of the compiled PDF using the todo command\todo{Here's a comment in the margin!}, as shown in the example on the right. You can also add inline comments:

\todo[inline, color=green!40]{This is an inline comment.}

\subsection{How to add Tables}

Use the table and tabular commands for basic tables --- see Table~\ref{tab:widgets}, for example. 

\begin{table}
\centering
\begin{tabular}{l|r}
Item & Quantity \\\hline
Widgets & 42 \\
Gadgets & 13
\end{tabular}
\caption{\label{tab:widgets}An example table.}
\end{table}

\subsection{How to write Mathematics}

\LaTeX{} is great at typesetting mathematics. Let $X_1, X_2, \ldots, X_n$ be a sequence of independent and identically distributed random variables with $\text{E}[X_i] = \mu$ and $\text{Var}[X_i] = \sigma^2 < \infty$, and let
\[S_n = \frac{X_1 + X_2 + \cdots + X_n}{n}
      = \frac{1}{n}\sum_{i}^{n} X_i\]
denote their mean. Then as $n$ approaches infinity, the random variables $\sqrt{n}(S_n - \mu)$ converge in distribution to a normal $\mathcal{N}(0, \sigma^2)$.


\subsection{How to create Sections and Subsections}

Use section and subsections to organize your document. Simply use the section and subsection buttons in the toolbar to create them, and we'll handle all the formatting and numbering automatically.

\subsection{How to add Lists}

You can make lists with automatic numbering \dots

\begin{enumerate}
\item Like this,
\item and like this.
\end{enumerate}
\dots or bullet points \dots
\begin{itemize}
\item Like this,
\item and like this.
\end{itemize}

\subsection{How to add Citations and a References List}

You can upload a \verb|.bib| file containing your BibTeX entries, created with JabRef; or import your \href{https://www.overleaf.com/blog/184}{Mendeley}, CiteULike or Zotero library as a \verb|.bib| file. You can then cite entries from it, like this: %\cite{greenwade93}. Just remember to specify a bibliography style, as well as the filename of the \verb|.bib|.

You can find a \href{https://www.overleaf.com/help/97-how-to-include-a-bibliography-using-bibtex}{video tutorial here} to learn more about BibTeX.

We hope you find Overleaf useful, and please let us know if you have any feedback using the help menu above --- or use the contact form at \url{https://www.overleaf.com/contact}!

==> unused.tex <==
% 1 table for 4 simulations (workload, service level, pickup time, drive to the charger time)
% v=30mph, /4
\subsubsection{Scenario 1: Higher Velocity and Lower Charger Parameter}

\noindent This scenario uses the fixed parameters outlined in Table \ref{table:fixed_parameters}. %The variable parameters in Table \ref{table:variable_parameters} are set as described below. 
The simulation duration and end time differ for each section and are detailed further. The average velocity of the EVs is set at a high value of 30 mph. The number of chargers is matched to the number of EVs requiring charging to maintain consistent SoCs. In certain simulations, the number of chargers is reduced to analyze the impact of limited charging availability.
% determined using the formula: number of chargers = (fleet size * consumption * average velocity / charge rate) /4. 
The charging algorithm employed in this scenario is the ``charge idle cars all the time'' algorithm, as described in Section \ref{sec: match_charge}. Various simulations explore different different matching algorithms, as specified in the corresponding sections.

\vspace{0.2cm}
\noindent \textbf{One-day simulations:} The simulations in this section have a duration of 1 day, ending on May 2, 2024, at 00:00:00. The fleet size is the same as peak trip demand.

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.25]{figures/Legend.png}
\end{figure}
\vspace{-0.5cm}
\begin{figure}[H]
    \centering
    \begin{minipage}[h]{0.3\textwidth}
        \centering
        \includegraphics[scale=0.35]{figures/1_day_d_1_high_velocity.png}
        \captionsetup{justification=centering, margin=0.1cm}
        \vspace{-0.5cm}
        \caption{1-day power-of-$1$ (closest dispatch)}
        \label{fig:1_day_d_1_high_velocity_new}
    \end{minipage}
    \hfill
    \begin{minipage}[h]{0.3\textwidth}
        \centering
        \includegraphics[scale=0.35]{figures/1_day_d_3_high_velocity.png}
        \captionsetup{justification=centering, margin=1cm}
        \vspace{-0.5cm}
        \caption{1-day power-of-$3$ dispatch}
        \label{fig:1_day_d_3_high_velocity_new}
    \end{minipage}
    \hfill
    \begin{minipage}[h]{0.3\textwidth}
        \centering
        \includegraphics[scale=0.35]{figures/1_day_d_5_high_velocity.png}
        \captionsetup{justification=centering, margin=1cm}
        \vspace{-0.5cm}
        \caption{1-day power-of-$5$ dispatch}
        \label{fig:1_day_d_5_high_velocity_new}
    \end{minipage}
\end{figure}

\begin{table}[h]
    \centering
    \vspace{-0.2cm}
    \begin{tabular}{ |p{3.7cm}|p{2.6cm}|p{2.6cm}|p{2.6cm}| }
        \hline
        Matching algorithm & closest dispatch & power-of-$3$  & power-of-$5$ \\
        \hline
        Average pickup time (mins) & 2.45 & 3.16 & 3.70\\
        \hline
        Average time to chargers (mins) & 5.24 & 5.42 & 5.41\\
        \hline
        Service level & 93.93\% & 96.77\% & 95.42\%\\
        \hline
        Workload served & 91.91\% & 94.09\% & 92.72\%\\
        \hline
    \end{tabular}
    \captionsetup{justification=centering}
    \caption{1-day simulations with average velocity of 30 mi/hr, fleet size of 1636, and a total of 141 chargers. The charging algorithm is ``charge idle cars all the time'' as described in Section \ref{sec: match_charge}.}
    \label{table:1_day_high_velocity_low_charger}
\end{table}

\noindent In this section, we test the performance of the power-of-$d$ vehicles dispatch policy for $d \in \{1, 3, 5\}$. Our insights are consistent with that of \cite{varma_ev}.

\noindent \textbf{Comparison of Power-of-$d$ Vehicle Dispatch Algorithms with Different $d$ in 1-day Simulation:}

\noindent First, using power-of-$1$ vehicle dispatch algorithm (i.e., closest vehicle dispatch), as illustrated in Fig. \ref{fig:1_day_d_1_high_velocity_new}, nearly all trip demands are met during the first two-thirds of the time period, and this is indicated by the substantial blue area almost completely filling the space beneath the pink line. However, a noticeable decline in performance occurs in the final third of the period, which is represented by an expansion in the orange area (vehicles in pickup mode) and the larger green region (idle vehicles). In other words, the algorithm drops the incoming trips while there are EVs idling. Such a behavior arises because a small $d$ value restricts consideration to the nearest EV for each customer. For each incoming customer, only the closest EV is considered, and the customer is dropped if that EV has a low SoC. Thus, while other nearby EVs might have adequate SoC, we still do not serve the customer. This suggests that increasing the value of $d$ could enhance performance by broadening the selection pool of candidate vehicles.
% The average SoC curve shows a rapid decline during peak daytime hours due to increased trip demands. In contrast, during periods of low demand at night, the average SoC swiftly bounces back, indicated by the substantial yellow region (vehicle charging) and ascending SoC curve overnight.
%\noindent The dynamics between the green area (idle vehicles) and orange area (vehicles in pickup) represent a balance between two competing factors. Increasing $d$ enlarges the orange region and diminishes the green area due to prolonged pickup times. To enhance system efficiency, a reduction in the green area is desirable. Initially, 
As $d$ increases, the number of trips served rises, as shown by the enlarged blue region in Fig. \ref{fig:1_day_d_3_high_velocity_new}. However, overly high $d$ values can result in diminished performance, as indicated in Fig. \ref{fig:1_day_d_5_high_velocity_new}. In particular, if the value of $d$ is too high, the increase in pickup times results in a smaller proportion of customers served. Determining the optimal value of $d$ involves evaluating the trade-off between minimizing pickup times and balancing the load across the fleet. A strategy that minimizes pickup time results in a smaller orange region but potentially increases the green area, as shown by the closest vehicle dispatch algorithm in Fig. \ref{fig:1_day_d_1_high_velocity_new}. In contrast, balancing the load across the fleet reduces the green area, aiming to minimize the number of idle vehicles when many trips are getting dropped. An optimal dispatch strategy would aim to minimize idle vehicles while efficiently handling trip demands without spending too much time picking up customers.

\noindent Among the three tested power-of-$d$ simulations in this scenario, the power-of-$3$ vehicle dispatch algorithm yields the best performance, achieving the highest service level and workload efficiency, as shown in Table \ref{table:1_day_high_velocity_low_charger}. This approach adopts a comprehensive approach by evaluating the three closest vehicles and selecting the one with the highest SoC for each trip request. By doing so, it reduces the number of idle vehicles, increases the total number of trips served, and enhances active pickups. Meanwhile, unlike the power-of-5 algorithm, which sacrifices efficiency due to increased pickup delays, the power-of-3 strategy does not consider too many closest vehicles which potentially increase the average pickup distance and time too much. Therefore, it achieves a balanced and effective performance.

\vspace{0.2cm}
\noindent \textbf{Three-day simulations:} The simulations in this section have a duration of 3 days, ending on May 4, 2024, at 00:00:00. The fleet size is set to be 80\% of peak trip demand.

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.25]{figures/Legend.png}
\end{figure}
\vspace{-0.5cm}
\begin{figure}[H]
    \centering
    \begin{minipage}[h]{0.32\textwidth}
        \centering
        \includegraphics[scale=0.33]{figures/3_day_CAD_high_velocity_n_chargers_0.25_new.png}
        \captionsetup{justification=centering, margin=0.3cm}
        \vspace{-0.5cm}
        \caption{3-day closest available dispatch with v=30mph and less chargers}
        \label{fig:3_day_CAD_high_velocity_n_chargers_0.25_new}
    \end{minipage}
    \hfill
    \begin{minipage}[h]{0.32\textwidth}
        \centering
        \includegraphics[scale=0.33]{figures/3_day_d_1_high_velocity_n_chargers_0.25_new.png}
        \captionsetup{justification=centering, margin=0.3cm}
        \vspace{-0.5cm}
        \caption{3-day power-of-$1$ (closest dispatch) with v=30mph and less chargers}
        \label{fig:3_day_d_1_high_velocity_n_chargers_0.25_new}
    \end{minipage}
    \hfill
    \begin{minipage}[h]{0.32\textwidth}
        \centering
        \includegraphics[scale=0.33]{figures/3_day_d_5_high_velocity_n_chargers_0.25_new.png}
        \captionsetup{justification=centering, margin=0.3cm}
        \vspace{-0.5cm}
        \caption{3-day power-of-$5$ with v=30mph and less chargers}
        \label{fig:3_day_d_5_high_velocity_n_chargers_0.25_new}
    \end{minipage}
\end{figure}

\begin{table}[h]
    \centering
    \vspace{-0.2cm}
    \begin{tabular}{ |p{3.1cm}|p{2.5cm}|p{2.5cm}|p{2.2cm}|p{2.1cm}|p{2.1cm}|p{2.1cm}| }
        \hline
        % \multicolumn{5}{|c|}{3-day Simulations with Higher Velocity and Lower Charger Parameter} \\
        % \hline
        % \hline
        Matching algorithm & closest available & closest dispatch & power-of-$3$ & power-of-$5$ & power-of-$10$\\
        % \hline
        % Charging algorithm & charge idle cars all the time & charge idle cars all the time & charge idle cars all the time & charge idle cars all the time\\
        % \hline
        % Average velocity (mph) & 30 & 30 & 30 & 30\\
        % \hline
        % Fleet size & 2101 & 2101 & 2101 & 2101\\
        % \hline
        % Number of chargers & 181 & 181 & 181 & 181\\
        \hline
        Average pickup time (mins) & 3.07 & 2.55 & 3.46 & 3.77 & 4.23\\
        \hline
        Average time to chargers (mins) & 4.98 & 4.27 & 5.29 & 5.17 & 4.94\\
        \hline
        Service level & 96.04\% & 89.90\% & 92.97\% & 93.14\% & 93.00\%\\
        \hline
        Workload served & 93.54\% & 87.83\% & 90.36\% & 90.64\% & 90.40\%\\
        \hline
    \end{tabular}
    \captionsetup{justification=centering}
    \caption{3-day simulations with average velocity of 30 mi/hr, fleet size of 1680, and a total of 144 chargers. The charging algorithm is ``charge idle cars all the time'' as described in Section \ref{sec: match_charge}.}
    \label{table:3_day_high_velocity_low_charger}
\end{table}

\noindent Although the power-of-$5$ vehicle dispatch algorithm has a higher average pickup and driving times to chargers compared to the power-of-$1$ (closest dispatch) algorithm, as shown in Table \ref{table:3_day_high_velocity_low_charger}, it significantly improves service levels and workload. By considering a broader selection of vehicles and choosing the one with the highest SoC for each trip request, the power-of-$5$ algorithm effectively reduces idle vehicles and increases active pickups, especially toward the end of the simulation. Consequently, in Fig. \ref{fig:3_day_d_1_high_velocity_n_chargers_0.25_new}, the original green area (representing idleness) and the orange area (representing driving to chargers) under the pink curve are replaced by an expanded blue area (served trips) in Fig. \ref{fig:3_day_d_5_high_velocity_n_chargers_0.25_new}. The increase in workload leads to higher charging activities, represented by the larger yellow area in Fig. \ref{fig:3_day_d_5_high_velocity_n_chargers_0.25_new}. In this way, the average SoC of vehicles using the power-of-$5$ algorithm drops faster than that of the power-of-$1$ by the end of the simulation. Additionally, the power-of-$10$ algorithm incurs the longest pickup times, which slightly lowers its service level and workload efficiency compared to the power-of-$5$ approach.

\noindent The three-day simulations are all conducted at a high custom-defined vehicle velocity of 30 mph with fewer charging stations. Among these simulations, the closest available dispatch algorithm achieves the highest service level and workload. While both the closest available dispatch algorithm and power-of-$5$ algorithm perform similarly, the former serves more trips during peak demand periods. Specifically, the blue area in Fig. \ref{fig:3_day_CAD_high_velocity_n_chargers_0.25_new} around time = 3800 mins is larger compared to Fig. \ref{fig:3_day_d_5_high_velocity_n_chargers_0.25_new}, which is the main difference of their performances. The advantage of the closest available dispatch algorithm lies in its ability to minimize pickup time and distance by selecting the nearest available vehicle, especially when the average SoC remains sufficiently high. Therefore, choosing the closest available vehicle or the one with the highest SoC among the five closest ones does not differ a lot. In contrast, the power-of-$5$ algorithm may unnecessarily delay pickups by choosing a much farther vehicle with a marginally higher SoC, which is not always beneficial. This is reflected in Fig. \ref{fig:3_day_d_5_high_velocity_n_chargers_0.25_new}, where the larger orange area indicates more time spent driving to pickup locations during the peak demand. Overall, the closest available dispatch algorithm outperforms the power-of-$5$ algorithm in this scenario.



% low velocity vs. high velocity
\noindent Comparing the simulation results in Table \ref{table:3_day_low_velocity_low_charger} and Table \ref{table:3_day_high_velocity_low_charger} under identical policies and parameters highlights the significant impact of lower average velocity of vehicles. In the low-velocity scenario, both the average pickup time and the time required to reach charging stations are considerably higher. The higher-velocity scenario for the closest dispatch policy demonstrates greater efficiency, as vehicles are able to pick up passengers and reach charging stations more quickly. This improvement is reflected in Table \ref{table:3_day_high_velocity_low_charger}, which shows substantially reduced average pickup time and average time driving to chargers, as well as in Fig. \ref{fig:3_day_d_1_high_velocity_n_chargers_0.25_new}, where the smaller orange and purple areas represent fewer vehicles engaged in picking up customers and driving to chargers. Conversely, in the low-velocity scenario for closest dispatch shown in Fig. \ref{fig:3_day_d_1_low_velocity_n_chargers_0.25_new}, the orange and purple areas are largely expanded. As a result, the fleet is less capable of handling trip requests at lower velocities, as indicated by the diminished blue area (served trip) in the figures. This results in a noticeable decline in the overall service level and workload.

\noindent Additionally, the combination of low average vehicle velocity and a limited number of chargers lead to a consistent decline in the overall average SoC throughout the three-day simulation period. Unlike the high-velocity scenario in the previous section, where the average SoC could fully recover, in the low-velocity section, the average SoC fails to return to its initial level by the third day. This leads to a gradual degradation in performance over time.

